Privacy Impact Assessment: Comparing methodologies with a focus on practicality

Privacy and data protection have become more and more important in recent years since an increasing number of enterprises and startups are harvesting personal data as a part of their business model. One central requirement of the GDPR is the implementation of a data protection impact assessment for privacy critical systems. However, the law does not dictate or recommend the use of any particular framework. In this paper we compare different data protection impact assessment frameworks. We have developed a comparison and evaluation methodology and applied this to three popular impact assessment frameworks. The result of this comparison shows the weaknesses and strengths, but also clearly indicates that none of the tested frameworks fulfill all desired properties. Thus, the development of a new or improved data protection impact assessment framework is an important open issue for future work, especially for sector specific applications.

==> rand <==

@misc{kristof_van_quathem_google_2019,
	title = {Google fined {EUR} 50 million in {France} for {GDPR} violation},
	url = {https://www.insideprivacy.com/eu-data-protection/google-fined-e50-million-in-france-for-gdpr-violation/},
	abstract = {On January 21, 2019, the French Supervisory Authority for data protection (“CNIL”) issued a fine of €50 million against Google for violations of the},
	language = {en-US},
	urldate = {2019-07-26},
	journal = {Inside Privacy},
	author = {{Kristof Van Quathem} and {Jetty Tielemans} and {Anna Oberschelp de Meneses} and {Nicholas Shepherd}},
	month = jan,
	year = {2019},
	file = {Snapshot:D\:\\Benutzer\\Zotero\\storage\\JA3DJRBF\\google-fined-e50-million-in-france-for-gdpr-violation.html:text/html}
}

@misc{zen_soo_alibabas_2019,
	title = {Alibaba’s {Jack} {Ma} says he is ‘worried’ {Europe} will stifle innovation with too much tech regulation {\textbar} {South} {China} {Morning} {Post}},
	url = {https://www.scmp.com/tech/big-tech/article/3010606/alibabas-jack-ma-says-he-worried-europe-will-stifle-innovation-too},
	urldate = {2019-07-26},
	author = {{Zen Soo}},
	month = may,
	year = {2019},
	file = {Alibaba’s Jack Ma says he is ‘worried’ Europe will stifle innovation with too much tech regulation | South China Morning Post:D\:\\Benutzer\\Zotero\\storage\\Y6Y5R24E\\alibabas-jack-ma-says-he-worried-europe-will-stifle-innovation-too.html:text/html}
}

@misc{noauthor_pias_2017,
	title = {{PIAs} and {GDPR} {DPIAs} – {A} {Best} {Practice} {Guide}},
	url = {https://www.corporatecomplianceinsights.com/pias-gdpr-dpias-best-practice-guide/},
	abstract = {Under the GDPR, a significant new change is a requirement for companies to conduct Data Protection Impact Assessments for high-risk processing activities.},
	language = {en-US},
	urldate = {2019-07-26},
	journal = {Corporate Compliance Insights},
	month = dec,
	year = {2017},
	file = {Snapshot:D\:\\Benutzer\\Zotero\\storage\\TDQIU9S2\\pias-gdpr-dpias-best-practice-guide.html:text/html}
}

@article{noauthor_cnil_2018,
	title = {{CNIL} {PIA}},
	language = {en},
	year = {2018},
	pages = {109},
	file = {2018 - PIA, knowledge bases.pdf:D\:\\Benutzer\\Zotero\\storage\\VKQ93KQP\\2018 - PIA, knowledge bases.pdf:application/pdf;cnil-pia-1-en-methodology.pdf:D\:\\Benutzer\\Zotero\\storage\\DC5RKVMX\\cnil-pia-1-en-methodology.pdf:application/pdf;cnil-pia-2-en-templates.pdf:D\:\\Benutzer\\Zotero\\storage\\KDHIX6Z7\\cnil-pia-2-en-templates.pdf:application/pdf}
}

@misc{14:00-17:00_iso/iec_nodate,
	title = {{ISO}/{IEC} 29134:2017},
	shorttitle = {{ISO}/{IEC} 29134},
	url = {http://www.iso.org/cms/render/live/en/sites/isoorg/contents/data/standard/06/22/62289.html},
	abstract = {Information technology -- Security techniques -- Guidelines for privacy impact assessment},
	language = {en},
	urldate = {2019-06-27},
	journal = {ISO},
	author = {{14:00-17:00}},
	file = {Snapshot:D\:\\Benutzer\\Zotero\\storage\\SWZFKFWP\\62289.html:text/html}
}

@inproceedings{veseli_engineering_2019,
	address = {Limassol, Cyprus},
	title = {Engineering privacy by design: lessons from the design and implementation of an identity wallet platform},
	isbn = {978-1-4503-5933-7},
	shorttitle = {Engineering privacy by design},
	url = {http://dl.acm.org/citation.cfm?doid=3297280.3297429},
	doi = {10.1145/3297280.3297429},
	language = {en},
	urldate = {2019-06-27},
	booktitle = {Proceedings of the 34th {ACM}/{SIGAPP} {Symposium} on {Applied} {Computing}  - {SAC} '19},
	publisher = {ACM Press},
	author = {Veseli, Fatbardh and Olvera, Jetzabel Serna and Pulls, Tobias and Rannenberg, Kai},
	year = {2019},
	pages = {1475--1483},
	file = {Veseli et al. - 2019 - Engineering privacy by design lessons from the de.pdf:D\:\\Benutzer\\Zotero\\storage\\4CWCYC83\\Veseli et al. - 2019 - Engineering privacy by design lessons from the de.pdf:application/pdf}
}

@article{cavoukian_information_nodate,
	title = {Information \& {Privacy} {Commissioner} {Ontario}, {Canada}},
	language = {en},
	author = {Cavoukian, Dr Ann},
	pages = {6},
	file = {Cavoukian - Information & Privacy Commissioner Ontario, Canada.pdf:D\:\\Benutzer\\Zotero\\storage\\E5M4VRN9\\Cavoukian - Information & Privacy Commissioner Ontario, Canada.pdf:application/pdf}
}

@article{wright_comparative_2013,
	title = {A {Comparative} {Analysis} of {Privacy} {Impact} {Assessment} in {Six} {Countries}},
	volume = {9},
	abstract = {The European Commission is revising the EU’s data protection framework. One of the changes concerns privacy impact assessment (PIA). This paper argues that the European Commission and the EU Member States should draw on the experience of other countries that have adopted PIA policies and methodologies to construct its own framework. There are similarities and differences in the approaches of Australia, Canada, Ireland, New Zealand, the UK and US, the countries with the most experience in PIA. Each has its strong points, but also shortcomings. Audits have identified some of the latter in the instance of Canada. This paper provides a comparative analysis of the six countries to identify some of the best elements that could be used to improve Article 33 in European Commission’s proposed Data Protection Regulation.},
	language = {en},
	number = {1},
	author = {Wright, David and Finn, Rachel and Rodrigues, Rowena},
	year = {2013},
	pages = {21},
	file = {Wright et al. - 2013 - A Comparative Analysis of Privacy Impact Assessmen.pdf:D\:\\Benutzer\\Zotero\\storage\\JB5VD7QI\\Wright et al. - 2013 - A Comparative Analysis of Privacy Impact Assessmen.pdf:application/pdf}
}

@misc{noauthor_privacy_nodate,
	title = {Privacy {Impact} {Assessment} ({PIA}) {\textbar} {CNIL}},
	url = {https://www.cnil.fr/en/PIA-privacy-impact-assessment-en},
	urldate = {2019-06-27},
	file = {Privacy Impact Assessment (PIA) | CNIL:D\:\\Benutzer\\Zotero\\storage\\IQE7PKD7\\PIA-privacy-impact-assessment-en.html:text/html}
}

@inproceedings{ahmadian_privacy-enhanced_2019,
	address = {Limassol, Cyprus},
	title = {Privacy-enhanced system design modeling based on privacy features},
	isbn = {978-1-4503-5933-7},
	url = {http://dl.acm.org/citation.cfm?doid=3297280.3297431},
	doi = {10.1145/3297280.3297431},
	abstract = {To ensure that their stakeholders’ privacy concerns are addressed systematically from the early development phases, organizations can perform a privacy enhancement of the system design, in which appropriate technical and organizational controls are established. Such a privacy enhancement needs to account for three crucial types of input: First, risks to the rights of natural persons, as determined in a dedicated privacy impact assessment. Second, potential interrelations and dependencies among the privacy controls. Third, potential trade-offs regarding the costs of the controls. Despite numerous existing privacy enhancing technologies and catalogs of privacy controls, there has been no systematic methodology to support privacy enhancement based on these types of input.},
	language = {en},
	urldate = {2019-06-27},
	booktitle = {Proceedings of the 34th {ACM}/{SIGAPP} {Symposium} on {Applied} {Computing}  - {SAC} '19},
	publisher = {ACM Press},
	author = {Ahmadian, Amir Shayan and Strüber, Daniel and Jürjens, Jan},
	year = {2019},
	pages = {1492--1499},
	file = {Ahmadian et al. - 2019 - Privacy-enhanced system design modeling based on p.pdf:D\:\\Benutzer\\Zotero\\storage\\GDEED7UG\\Ahmadian et al. - 2019 - Privacy-enhanced system design modeling based on p.pdf:application/pdf}
}

@article{iwaya_engineering_nodate,
	title = {Engineering {Privacy} for {Mobile} {Health} {Data} {Collection} {Systems} in the {Primary} {Care}},
	abstract = {Mobile health (mHealth) systems empower Community Health Workers (CHWs) around the world, by supporting the provisioning of CommunityBased Primary Health Care (CBPHC) – primary care outside the health facility into people’s homes. In particular, Mobile Health Data Collection Systems (MDCSs) are used by CHWs to collect health-related data about the families that they treat, replacing paper-based approaches for health surveys. Although MDCSs signiﬁcantly improve the overall eﬃciency of CBPHC, existing and proposed solutions lack adequate privacy and security safeguards. In order to bridge this knowledge gap between the research areas of mHealth and privacy, the main research question of this thesis is: How to design secure and privacypreserving systems for Mobile Health Data Collection Systems? To answer this question, the Design Method is chosen as an engineering approach to analyse and design privacy and security mechanisms for MDCSs. Among the main contributions, a comprehensive literature review of the Brazilian mHealth ecosystem is presented. This review led us to focus on MDCSs due to their impact on Brazil’s CBPHC, the Family Health Strategy programme. On the privacy engineering side, the contributions are a Privacy Impact Assessment (PIA) for the GeoHealth MDCS and three mechanisms: (a) SecourHealth, a security framework for data encryption and user authentication; (b) an Ontology-based Data Sharing System (O-DSS) that provides obfuscation and anonymisation functions; and, (c) an electronic consent (e-Consent) tool for obtaining and handling informed consent. Additionally, practical experience is shared about designing a MDCS, GeoHealth, and deploying it in a largescale experimental study. In conclusion, the contributions of this thesis oﬀer guidance to mHealth practitioners, encouraging them to adopt the principles of privacy by design and by default in their projects.},
	language = {en},
	author = {Iwaya, Leonardo Horn},
	pages = {274},
	file = {Iwaya - Engineering Privacy for Mobile Health Data Collect.pdf:D\:\\Benutzer\\Zotero\\storage\\9W25IDZZ\\Iwaya - Engineering Privacy for Mobile Health Data Collect.pdf:application/pdf}
}

@article{gruschka_privacy_nodate,
	title = {Privacy {Issues} and {Data} {Protection} in {Big} {Data} {A} {Use} {Case} {Analysis} under {GDPR}},
	abstract = {Big data has become a great asset for many organizations, promising improved operations and new business opportunities. However, big data has increased access to sensitive information that when processed can directly jeopardize the privacy of individuals and violate data protection laws. As a consequence, data controllers and data processors may be imposed tough penalties for non-compliance that can result even to bankruptcy. In this paper we discuss the current state of the legal regulations and analyze different data protection and privacy preserving techniques in the context of big data analysis. In addition, we present and analyze two real-life research projects as use-cases dealing with sensitive data and actions to comply with the data regulation laws. We show which types of information might become a privacy risk, the employed privacy preserving techniques in accordance to the legal requirements and the inﬂuence of these techniques on the data processing phase and the research results.},
	language = {en},
	author = {Gruschka, Nils and Mavroeidis, Vasileios and Vishi, Kamer and Jensen, Meiko},
	pages = {7},
	file = {Gruschka et al. - Privacy Issues and Data Protection in Big Data A U.pdf:D\:\\Benutzer\\Zotero\\storage\\IWPES45I\\Gruschka et al. - Privacy Issues and Data Protection in Big Data A U.pdf:application/pdf}
}

@incollection{hansen_data_2018,
	address = {Cham},
	title = {Data {Protection} {Impact} {Assessment}: {A} {Hands}-{On} {Tour} of the {GDPR}’s {Most} {Practical} {Tool}},
	volume = {526},
	isbn = {978-3-319-92924-8 978-3-319-92925-5},
	shorttitle = {Data {Protection} {Impact} {Assessment}},
	url = {http://link.springer.com/10.1007/978-3-319-92925-5_13},
	abstract = {This workshop introduced participants to the process of Data Protection Impact Assessment. This new tool of the GDPR is highly relevant for any processing of personal data, as it helps to structure the process, be aware of data protection issues and the relevant legislation and implement proper safeguards to protect data subjects. For processing operations posing a high risk for data subjects, a DPIA is mandatory from May 2018. The interactive workshop provided a framework for DPIA and guidance on specific questions such as when a high risk is likely to occur or how specific risks can be evaluated, which was assessed by participants in an interactive session with two different scenarios.},
	language = {en},
	urldate = {2019-06-27},
	booktitle = {Privacy and {Identity} {Management}. {The} {Smart} {Revolution}},
	publisher = {Springer International Publishing},
	author = {Bieker, Felix and Martin, Nicholas and Friedewald, Michael and Hansen, Marit},
	editor = {Hansen, Marit and Kosta, Eleni and Nai-Fovino, Igor and Fischer-Hübner, Simone},
	year = {2018},
	doi = {10.1007/978-3-319-92925-5_13},
	pages = {207--220},
	file = {Bieker et al. - 2018 - Data Protection Impact Assessment A Hands-On Tour.pdf:D\:\\Benutzer\\Zotero\\storage\\YVRWEKT8\\Bieker et al. - 2018 - Data Protection Impact Assessment A Hands-On Tour.pdf:application/pdf}
}

@article{noauthor_linddun_tutorial_nodate,
	title = {{LINDDUN}\_tutorial},
	language = {en},
	pages = {36},
	file = {LINDDUN_tables.pdf:D\:\\Benutzer\\Zotero\\storage\\KFGRRSTQ\\LINDDUN_tables.pdf:application/pdf;LINDDUN_tutorial.pdf:D\:\\Benutzer\\Zotero\\storage\\UMF8Q6MQ\\LINDDUN_tutorial.pdf:application/pdf;Privacy threat tree modeling:D\:\\Benutzer\\Zotero\\storage\\22B4339V\\CW675.pdf:application/pdf}
}

@article{european_parliament_&_council_regulation_2016,
	title = {Regulation ({EU}) 2016/679 -- {Regulation} on the protection of natural persons with regard to the processing of personal data and on the free movement of such data, and repealing {Directive} 95/46/{EC} ({General} {Data} {Protection} {Regulation})},
	volume = {L119},
	number = {4.5.2016},
	journal = {Official Journal of the European Union},
	author = {{European Parliament \& Council}},
	month = apr,
	year = {2016},
	pages = {1--88}
}
